Environment Generation for Zero-Shot Compositional Reinforcement Learning

Many real-world problems are compositional - solving them requires completing interdependent sub-tasks, either in series or in parallel, that can be represented as a dependency graph. Deep reinforcement learning (RL) agents often struggle to learn such complex tasks due to the long time horizons and sparse rewards. To address this problem, we present Compositional Design of Environments (CoDE), which trains a Generator agent to automatically build a series of compositional tasks tailored to the RL agent's current skill level. This automatic curriculum not only enables the agent to learn more complex tasks than it could have otherwise, but also selects tasks where the agent's performance is weak, enhancing its robustness and ability to generalize zero-shot to unseen tasks at test-time. We analyze why current environment generation techniques are insufficient for the problem of generating compositional tasks, and propose a new algorithm that addresses these issues. Our results assess learning and generalization across multiple compositional tasks, including the real-world problem of learning to navigate and interact with web pages. We learn to generate environments composed of multiple pages or rooms, and train RL agents capable of completing wide-range of complex tasks in those environments. We contribute two new benchmark frameworks for generating compositional tasks, compositional MiniGrid and gMiniWoB for web navigation.CoDE yields 4x higher success rate than the strongest baseline, and demonstrates strong performance of real websites learned on 3500 primitive tasks.

==> src/background.tex <==
%\vspace*{-0.1in}
\section{Background on Web Navigation Problem}
\label{sec:background}
%\vspace*{-0.02in}
%\subsection{Web Navigation Problem}
Following previous work \citep{shi2017world,gur2018learning,liu2018reinforcement}, we formulate web navigation as a sequential decision making problem where we train an agent, parameterized by a network $\pi(a_t | s_t; \Theta_i)$, that maps an input state $s_t$ to output action distribution to maximize the cumulative discounted reward, .i.e.,  $O=\sum_{t=0}^{T}{\gamma^t r_t}$ where $r_t$ is the reward at time step $t$, $\gamma$ is a discount factor, and $T$ is the length of an episode.
We use the web page and user instruction as the input state. The web page is dynamically updated at each time step, while the instruction is fixed at the beginning of an episode.
We represent web pages using Document Object Model (DOM), a tree of elements in a page, where each element is denoted by a set of (attribute, value) pairs and an array of features (such as spatial coordinates).
Instructions are given as a set of fields where each field is a (key, value) pair.
Keys are fixed for each task and values dynamically change based on user input.

Each action is represented as a tuple (element, field) that denotes acting on the element using the field as an input; i.e. typing the value of the field into the element.
% Different from previous works, we use a rule-based option to execute the action, such as 'clicking on a text box with user name'.
Agents receive a task success reward (1.0 or -1.0) at the end of each episode, a potential-based reward when the value of an element in the page is updated, and a small penalty each timestep to encourage efficient navigation.
As an example, consider a flight booking task where the agent is given an instruction \{\texttt{"Departure Date": "Friday", Destination Airport: "Los Angeles (LAX)"}\}.
The agent first picks a field (e.g. destination airport) and finds the corresponding text box in the page; then the corresponding value (``Los Angeles (LAX)") typed in to the text box.
If this value is correct, the agent receives a positive reward of $1 /  2 $ where $2$ is the number of fields in the instruction.

% \subsection{Protagonist Antagonist Induced Regret Environment Design (PAIRED)}
% Adversarial Environment Generation (AEG) trains an adversary policy $\pi_E$ to design environments to minimize the performance of an agent's policy, $\pi_P$. Let $R^P_i = \sum_{t=1}^T\gamma^tr_t^P$ be the total reward received by the agent for trajectory $i$. PAIRED \citep{dennis2020emergent} trains the adversary to maximize the agent's \textit{regret}, which is defined as the difference between the agent's return and the return of the optimal policy, $R^*-R^P$. To estimate the regret, PAIRED
% introduces a third agent, the \textit{antagonist} (with policy $\pi_A$), and  constrains the adversary to only generate feasible environments which the antagonist can complete. 
% % When the adversary generates an environment, both the protagonist and antagonist collect a trajectory and the difference between the total rewards $R(\tau^A)$ and $R(\tau^P)$ is the regret:
% % %
% % \begin{align}
% %     \textsc{Regret} = R(\tau^A) - R(\tau^P)
% %     \label{eq:paired_regret}
% % \end{align}
% When the adversary generates an environment $E$, both the protagonist and antagonist collect $M$ trajectories with returns $R^P_{1},...,R^P_{M}, R^A_{1},...,R^A_{M}$ in $E$. The regret is then estimated as:
% \begin{align}
%     \textsc{Regret} = \max_i R^A_i - \frac{1}{M}\sum_{m=1}^M R^P_m
%     \label{eq:paired_regret}
% \end{align}

% If the antagonist fails to surpass the protagonist, or reaches a local optimum, then the adversary cannot continue to learn as the REGRET becomes uninformative. In Section \ref{sec:loss_functions} we propose an improved objective which addresses this problem. 



==> src/background_before_rebuttal.tex <==
\section{Background}
% We will first assume that a website and a user instruction are a priori given and describe the web navigation problem accordingly, which will set the stage for the zero-shot generalization problem.

\subsection{Web Navigation Problem}
% Following the previous work \citep{shi2017world,gur2018learning,liu2018reinforcement}, we formulate the web navigation problem as a sequential decision making in a partially observable markov decision process (POMDP) which is a tuple $(S, O, A, \mathcal{T}, \mathcal{R}, \lambda)$ where $S$ is a set of states, $O$ is a set of observations, $A$ is a set of actions, $\mathcal{T}: S x A \longrightarrow S$ is a transition function, $R: S \longrightarrow \mathbb{R}$ is a reward function, and $\lambda$ is a discount factor.

Following previous work \citep{shi2017world,gur2018learning,liu2018reinforcement}, we formulate web navigation as a sequential decision making problem where we train an agent, parameterized by a network $\pi(a_t | s_t; \Theta_i)$, that maps an input state $s_t$ to output actions $a_t$ to maximize the cumulative discounted reward, .i.e.,  $O=\sum_{t=0}^{T}{\gamma^t r_t}$ where $r_t$ is the reward at time step $t$, $\gamma$ is a discount factor, and $T$ is the length of an episode.
We use the web page and user instruction as the input state. The web page is dynamically updated at each time step, while the instruction is fixed at the beginning of an episode.
We represent web pages using Document Object Model (DOM), a tree of elements in a page, where each element is denoted by a set of (attribute, value) pairs and an array of features (such as spatial coordinates).
Instructions are given as a set of fields where each field is a (key, value) pair.
Keys are fixed for each task and values dynamically change based on user input.

Each action is represented as a tuple (element, field) that denotes acting on the element using the field as an input; i.e. typing the value of the field into the element.
% Different from previous works, we use a rule-based option to execute the action, such as 'clicking on a text box with user name'.
Agents receive a task success reward (1.0 or -1.0) at the end of each episode, a potential-based reward when the value of an element in the page is updated, and a small penalty each timestep to encourage efficient navigation.
As an example, consider a flight booking task where the agent is given an instruction \{\texttt{"Departure Date": "Friday", Destination Airport: "Los Angeles (LAX)"}\}.
The agent first picks a field (e.g. destination airport) and finds the corresponding text box in the page; then the corresponding value (``Los Angeles (LAX)") typed in to the text box.
If this value is correct, the agent receives a positive reward of $1 /  N $ where $N$ is the number of fields.

% \textbf{States:} 
% % We represent a state at time step $t$ as a tuple $s_t=(W_t, I)$ where $W_t$ is a web page and $I$ is a user instruction given at the beginning of an episode.
% We use Document Object Model (DOM), a tree of elements in the page, as the observation of web pages.
% Each element ($e$) is denoted by a set of attibutes and their values (such as 'tag $\rightarrow$ input', 'value $\rightarrow$ ICLR2021') and an array of features (such as 'spatial coordinates').
% Instructions are given as a set of fields where each field ($f_t$) is a (key, value) pair.
% Keys are fixed for each task and values are dynamically generated by the user.
% An example profile for a \textit{Login} task would be \{\textit{"username"}: "iclr2021", \textit{"password"}: "1202rlci"\}.

% \textbf{Actions:} Actions are represented as a tuple $a=(e, f)$ that denotes acting on element $e$ using field $f$ as the input.
% We assume that there is a low level "option" that takes an action and executes a sequence of "clicks" and "types" on the corresponding element.

% \textbf{Rewards:} There are two types of rewards: (i) A binary task success that is retrieved only at the end of an episode and (ii) A potential based reward that is computed only when the value of an element in the page changes.
% For example, given \{\textit{"username"}: "iclr2021"\} and a text box on a web page, the corresponding option would type the value of the field into the text box.
% If this value is correct, we return a reward of $1 /  sizeof(I)$ where $sizeof(I)$ is the number of fields in the instruction; otherwise, we return minus this reward.
% This ensures that the maximum and minimum rewards that an agent can collect are bounded.

% \textbf{Transitions:} Transitions from one page to another are generated by events attached to elements.
% As an example, in Figure \ref{fig:rollout}, "Login and Checkout" has a POST event that validates user credentials and takes user to their checkout address form.

%Our main objective is to train a web navigation agent (WebNav) that maximizes the cumulative discounted reward over an episode, i.e., $O=\sum_{t=0}^{T}{r_t\lambda^t}$ where $r_t \in R$ and $T$ is the length of an episode.
%We assume that an agent $i$ is parameterized with a policy network $\pi^i(a_t | s_t; \Theta_i)$ that outputs a distribution over actions given a web page and a user instruction.
%An action is sampled from this distribution and sent to the environment to collect a reward and next web page state.

% \todo[inline]{I changed the policy notation to indicate the player using a superscript ($\pi^i$), so that it doesn't conflict with the t subscript ($r^i_t$) --NJ}

\subsection{Protagonist Antagonist Induced Regret Environment Design (PAIRED)}
Adversarial Environment Generation (AEG) trains an adversary policy $\pi_E$ to design environments to minimize the performance of an agent's policy, $\pi_P$. Let $R^P_i = \sum_{t=1}^T\gamma^tr_t^P$ be the total reward received by the agent for trajectory $i$. In minimax AEG, the objective for the adversary is simply: $-R^P$. Thus, minimax adversaries are incentivized to create excessively difficult or impossible environments, which may not enable the agent to learn. Instead, PAIRED \citep{dennis2020emergent} trains the adversary to maximize the agent's \textit{regret}, which is defined as the difference between the agent's return and the return of the optimal policy, $R^*-R^P$. When the reward function includes an incentive to complete the task more efficiently (which is true in our case), the regret will be highest for easy tasks which could be completed in a few steps by the optimal policy, but which the current policy fails to complete. Therefore, an adversary that maximizes the regret will continue to propose easier tasks until the agent begins to solve them, making regret a desirable objective for AEG.

To estimate the regret, PAIRED
introduces a third agent, the \textit{antagonist} (with policy $\pi_A$), and  constrains the adversary to only generate feasible environments which the antagonist can complete. 
% When the adversary generates an environment, both the protagonist and antagonist collect a trajectory and the difference between the total rewards $R(\tau^A)$ and $R(\tau^P)$ is the regret:
% %
% \begin{align}
%     \textsc{Regret} = R(\tau^A) - R(\tau^P)
%     \label{eq:paired_regret}
% \end{align}
When the adversary generates an environment $E$, both the protagonist and antagonist collect $M$ trajectories with returns $R^P_{1},...,R^P_{M}, R^A_{1},...,R^A_{M}$ in $E$. The regret is then estimated as:
\begin{align}
    \textsc{Regret} = \max_i R^A_i - \frac{1}{M}\sum_{m=1}^M R^P_m
    \label{eq:paired_regret}
\end{align}

As \citet{dennis2020emergent} show, if the adversary and antagonist coordinate and reach a Nash equilibrium with the protagonist, then the protagonist will have learned to minimize the regret. However, in practice gradient-based multi-agent RL has no convergence guarantees, is highly non-stationary, and will often fail to converge \citep{mazumdar2019policy,mazumdar2019finding}. If the antagonist and adversary in PAIRED fail to coordinate, then PAIRED minimizes regret with respect to the antagonist's policy. In that case, the objective in Equation \ref{eq:paired_regret} only forces the protagonist to learn to be as good as the antagonist. If the antagonist fails to improve, or reaches a local optimum, then the adversary cannot continue to train the protagonist. In Section \ref{sec:flexible} we propose an improved objective which addresses this problem. 

% As such, the regret will be highest if it is possible to obtain a high score in an environment, but the protagonist fails to do so.
% Because the protagonist and antagonist are initialized and trained together, the antagonist's score acts as a measure of the performance that a reasonable agent can obtain in the best case in a given environment.
%Because regret will be highest This objective leads the adversary to generate environments that challenge the protagonist, but are within the range of the agents' current skill level. 



==> src/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We acknowledge that our difficulty incentive based on the number or primitives may not always correlate with true task difficulty in Section \ref{sec:results}, and discuss further limitations in Appendix \ref{app:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{\textbf{See Appendix \ref{app:broader_impact}}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We state the reward assumption which is violated for the degenerate case proof in Section \ref{sec:failure_modes}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{\textbf{See Appendix \ref{app:reachprob}}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{\textbf{We open-sourced our code at \url{https://github.com/google-research/google-research/tree/master/compositional_rl}.}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{\textbf{Details about hyperparameters are given in the Appendix Section \ref{ap:adversary_network_details}}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{\textbf{Our plots include error bars of the confidence interval over five random seeds.}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Training CoDE was done on a single CPU for web environments and three CPUs with distributed training for the MiniGrid. Total training took about 7 days on web environments, and 5 days on MiniGrid. The code was implemented in Python, using Acme RL library with TF.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{\textbf{We build on and cite MiniGrid \cite{gym_minigrid}, MiniWoB \citep{shi2017world}, MiniWoB++ \citep{liu2018reinforcement}, ACME \cite{acme}, and TensorFlow \cite{tf}}}
  \item Did you mention the license of the assets?
    \answerYes{\textbf{ACME and TF are open sourced libraries.}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{\textbf{We are open-sourcing the code to support Adversarial Environment Generation.}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{\textbf{We do not use human subjects data.}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{\textbf{We do not use human subjects data.}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{\textbf{We do not use human subjects data.}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{\textbf{We do not use human subjects data.}}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{\textbf{We do not use human subjects data.}}
\end{enumerate}

\end{enumerate}

==> src/conclusion.tex <==
%\vspace*{-0.1in}
\section{Conclusion}
%\vspace*{-0.02in}
This work presents a novel technique for zero-shot generalization compositional task learning. We first formalized the compositional tasks with Petri Nets. Next we presented \adversary\, a generative architecture that creates new environments for \webnav\ agents to train on. The \adversary\ learns simultaneously two policies -- one adversarial making the environments challenging to the agents, and the second friendly lowering the difficult of the environments when the agents are not very proficient. In addition, we apply AEG to the problem of web navigation, and contribute an open-source environment that enables learning to design complex websites out of a set of compositional primitives. Our method is able to generate a curriculum of increasingly complicated websites, and successfully trains agents which can navigate challenging, high-dimensional websites. 


\ifdefined\isaccepted
\section*{Acknowledgements}
We thank Sungryull Sohn for providing help on Playground environments and discussions.
\fi

==> src/detailed_background.tex <==
\subsection{Protagonist Antagonist Induced Regret Environment Design (PAIRED)}
Adversarial Environment Generation (AEG) trains an adversary policy $\pi_E$ to design environments to minimize the performance of an agent's policy, $\pi_P$. Let $R^P_i = \sum_{t=1}^T\gamma^tr_t^P$ be the total reward received by the agent for trajectory $i$. In minimax AEG, the objective for the adversary is simply: $-R^P$. Thus, minimax adversaries are incentivized to create excessively difficult or impossible environments, which may not enable the agent to learn. Instead, PAIRED \citep{dennis2020emergent} trains the adversary to maximize the agent's \textit{regret}, which is defined as the difference between the agent's return and the return of the optimal policy, $R^*-R^P$. When the reward function includes an incentive to complete the task more efficiently (which is true in our case), the regret will be highest for easy tasks which could be completed in a few steps by the optimal policy, but which the current policy fails to complete. Therefore, an adversary that maximizes the regret will continue to propose easier tasks until the agent begins to solve them, making regret a desirable objective for AEG.

To estimate the regret, PAIRED
introduces a third agent, the \textit{antagonist} (with policy $\pi_A$), and  constrains the adversary to only generate feasible environments which the antagonist can complete. 
% When the adversary generates an environment, both the protagonist and antagonist collect a trajectory and the difference between the total rewards $R(\tau^A)$ and $R(\tau^P)$ is the regret:
% %
% \begin{align}
%     \textsc{Regret} = R(\tau^A) - R(\tau^P)
%     \label{eq:paired_regret}
% \end{align}
When the adversary generates an environment $E$, both the protagonist and antagonist collect $M$ trajectories with returns $R^P_{1},...,R^P_{M}, R^A_{1},...,R^A_{M}$ in $E$. The regret is then estimated as:
\begin{align}
    \textsc{Regret} = \max_i R^A_i - \frac{1}{M}\sum_{m=1}^M R^P_m
    \label{eq:paired_regret}
\end{align}

As \citet{dennis2020emergent} show, if the adversary and antagonist coordinate and reach a Nash equilibrium with the protagonist, then the protagonist will have learned to minimize the regret. However, in practice gradient-based multi-agent RL has no convergence guarantees, is highly non-stationary, and will often fail to converge \citep{mazumdar2019policy,mazumdar2019finding}. If the antagonist and adversary in PAIRED fail to coordinate, then PAIRED minimizes regret with respect to the antagonist's policy. In that case, the objective in Equation \ref{eq:paired_regret} only forces the protagonist to learn to be as good as the antagonist. If the antagonist fails to improve, or reaches a local optimum, then the adversary cannot continue to train the protagonist. In Section \ref{sec:loss_functions} we propose an improved objective which addresses this problem. 


% \subsection{Protagonist Antagonist Induced Regret Environment Design (PAIRED)}
% Adversarial Environment Generation (AEG) trains an adversary policy $\pi_E$ to design environments to minimize the performance of an agent's policy, $\pi_P$. Let $R^P_i = \sum_{t=1}^T\gamma^tr_t^P$ be the total reward received by the agent for trajectory $i$. PAIRED \citep{dennis2020emergent} trains the adversary to maximize the agent's \textit{regret}, which is defined as the difference between the agent's return and the return of the optimal policy, $R^*-R^P$. To estimate the regret, PAIRED
% introduces a third agent, the \textit{antagonist} (with policy $\pi_A$), and  constrains the adversary to only generate feasible environments which the antagonist can complete. 
% % When the adversary generates an environment, both the protagonist and antagonist collect a trajectory and the difference between the total rewards $R(\tau^A)$ and $R(\tau^P)$ is the regret:
% % %
% % \begin{align}
% %     \textsc{Regret} = R(\tau^A) - R(\tau^P)
% %     \label{eq:paired_regret}
% % \end{align}
% When the adversary generates an environment $E$, both the protagonist and antagonist collect $M$ trajectories with returns $R^P_{1},...,R^P_{M}, R^A_{1},...,R^A_{M}$ in $E$. The regret is then estimated as:
% \begin{align}
%     \textsc{Regret} = \max_i R^A_i - \frac{1}{M}\sum_{m=1}^M R^P_m
%     \label{eq:paired_regret}
% \end{align}

% If the antagonist fails to surpass the protagonist, or reaches a local optimum, then the adversary cannot continue to learn as the REGRET becomes uninformative. In Section \ref{sec:loss_functions} we propose an improved objective which addresses this problem. 


% \subsection{More on the PAIRED algorithm}
% Minimax adversaries are incentivized to create excessively difficult or impossible environments, which may not enable the agent to learn. Instead, PAIRED trains the adversary to maximize the REGRET, which is the difference between an antagonist (with policy $\pi_A$) and an protagonist (with policy $\pi_P$) agent's reward. When the reward function includes an incentive to complete the task more efficiently (which is true in our case), the regret will be highest for easy tasks which could be completed in a few steps by the optimal policy, but which the current policy fails to complete. Therefore, an adversary that maximizes the regret will continue to propose easier tasks until the agent begins to solve them, making regret a desirable objective for AEG.

% As \citet{dennis2020emergent} show, if the adversary and antagonist coordinate and reach a Nash equilibrium with the protagonist, then the protagonist will have learned to minimize the regret. However, in practice gradient-based multi-agent RL has no convergence guarantees, is highly non-stationary, and will often fail to converge \citep{mazumdar2019policy,mazumdar2019finding}. If the antagonist and adversary in PAIRED fail to coordinate, then PAIRED minimizes regret with respect to the antagonist's policy. In that case, the objective in Equation \ref{eq:paired_regret} only forces the protagonist to learn to be as good as the antagonist. If the antagonist fails to improve, or reaches a local optimum, then the adversary cannot continue to train the protagonist. In Section \ref{sec:loss_functions}, we propose an improved objective which addresses this problem. 



==> src/experiments.tex <==
%\vspace*{-0.1in}
\section{Evaluations}
%\vspace*{-0.02in}
\textbf{Evaluation setup:}
%\subsubsection{Test Environments}
We evaluate our models on MiniWoB \citep{shi2017world,liu2018reinforcement}, and a suite of environments implemented in gMiniWoB of varying difficulty levels using the same set of design primitives in gMiniWoB. These environments include `Login', `Enter Address', `Flight Booking', `Enter Payment', and `Shopping' websites. %, where the agents need to enter text or select information in the website while navigating between pages.
Each environment comes with 4 different difficulty levels by gradually adding more primitives.
These environments are never explicitly presented to agents during training, so performance in them measures how well agents can generalize to unseen websites at test time.

%\subsection{Navigator Agent Network Architecture}
% \textbf{Web Environment Design via PAIRED (\WEDP):}
% We initialize 2 independent antagonist and protagonist agents for web navigation.
\textbf{Agent architecture:} Following \citet{gur2018learning}, we utilize an LSTM based DOM tree encoder and a feed forward network to encode profile fields.
The \webnav\ agent policy outputs a joint distribution over elements and fields by measuring pairwise similarities between element encodings and profile fields.
We compute the state-value by using the marginal distribution of elements as attention weights over element encodings and passing the context vector through a FF network.
Web navigation agents are trained with an actor-critic algorithm \citep{liu2018reinforcement}.
We train the LSTM-based adversary network using \WEDP\ and \WEDPb\ with policy gradient (See Appendix \ref{ap:adversary_network_details} for more details on adversary policy network).

%\subsection{Baselines}
% We compare our models to several baseline methods including a curriculum learning method \citep{gur2018learning} that is shown to be very effective on web navigation tasks.
\textbf{Baselines:} We benchmark PAIRED, \WEDP, and \WEDPb\ against two additional baselines. First, a Domain Randomization (DR) agent, implemented using a similar approach as \citet{dennis2020emergent}.
After sampling the number of empty pages $k$ from a uniform distribution $U[0,K],$ we randomly sample a primitive (including SKIP), and a page from $U[0,k]$ for $N$ steps.
Second, a Curriculum Learning (CL) approach, which adapts the scheduled curriculum idea of \citet{gur2018learning} to zero-shot environment generation where we are not given a specific website but a set of design primitives.
We randomly sample each primitive w.r.t. a probability $p$ where $p$ is initialized with a small number and scheduled to reach $1.0$ during training.

% We also train with the budget enforcing approach (\WEDPb) and compare both models to above baselines.

\subsection{Results}
\begin{figure*}[tb]
\small
\centering
\vspace{-.2cm}
    \subfloat[Login]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/login.png}
    }%
    \subfloat[Address]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/address.png}
    }%
    \subfloat[Payment]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/payment.png}
    }\\%
    \vspace*{0.05in}
    \subfloat[Shopping]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/shopping.png}
    }%
    \subfloat[Flight booking]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/flight.png}
    }%
    \subfloat[Primitives]{\includegraphics[width=0.28\linewidth]{img/active_primitive_dist.png}\label{fig:primitivedistribution}}
    \caption{\small Comparison of PAIRED \citep{dennis2020emergent} and Flexible PAIRED with and without budget enforcing; averaged over 4 difficulty levels. (f): Percentage of active primitives over training steps (see Appendix \ref{ap:primitive_frequencies} for more details).}
    \label{fig:combinedpbt}
\end{figure*}

\begin{figure*}[tb]
\small
    \subfloat[Difficulty level 1]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/0.png}
    }%
    \subfloat[Difficulty level 2]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/1.png}
    }%
    \subfloat[Difficulty level 3]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/2.png}
    }%
    \subfloat[Difficulty level 4]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/3.png}
    }%
    \caption{\small Aggregated task success rate comparison of \WEDPb\ and baseline models on test environments with increasing difficulty levels. See Appendix \ref{ap:detailed-results} for detailed results.}
    \label{fig:tasksuccessaggregated}
    %\vspace{-.7cm}
\end{figure*}
\textbf{Importance of flexible \webnav\ agents}: Flexible \webnav\ agents learn better than the dedicated antagonist. We compare the b-PAIRED algorithm, which uses separate antagonist and protagonist agents, to the proposed \WEDPb\ algorithm that annotates the best performing agent as the antagonist.
%In Figure \ref{fig:combinedpbt}, we plot the performance of \WEDP\ against the original PAIRED, aggregated across difficulty levels.
\WEDPb\ improves upon b-PAIRED on all environments and continues to learn even when b-PAIRED struggles (Figure \ref{fig:combinedpbt}).
One reason is that when agents are separate and have very similar rewards, the regret becomes very small. This uninformative signal makes it difficult for the adversary to learn.
On the other hand, \WEDPb\ computes a consistently positive regret signal, which more clearly indicates to the \adversary\ which environments are challenging, but still feasible. 
The further ablation studies show that adding budget improves performance for both flexible, and original PAIRED method (see Appendix \ref{ap:miniwob} for MiniWoB studies and Appendix \ref{ap:weight_comp} for budget weight ablation).
%The rest of the experimental results use the \WEDP\ method.

%\subsection{Comparison on Test Environments}
\textbf{Importance of budget loss}: The budget objective significantly improves performance with \WEDPb\ outperforming \WEDP\ on test environments (Figure \ref{fig:tasksuccessaggregated}).
%We evaluate the performance of the proposed models and baselines on task success rate computed across test environments with different difficulty levels.
Further, both techniques significantly outperform the baseline models on all tasks, with \WEDPb\ effectively reaching more than 75\% task success across all difficulty levels.
Even as the complexity of the environments continues to increase (Section \ref{sec:complexity}), \WEDPb\ agents still perform consistently well without degrading performance.
While CL outperforms \WEDP\ early in the training, its performance drops significantly due to ignoring agents' skill level, and making environments that are too challenging for agents to complete.
We also observe that \WEDPb\ learns faster than \WEDP\ on all environments as \WEDPb\ reacts to agents' performance faster than \WEDP{} (Appendix \ref{ap:detailed-results}).

% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-0.5cm}
%   \begin{center}
%     \includegraphics[width=\linewidth]{img/active_primitive_dist.png}
%   \end{center}
%   \caption{Percentage of active primitives over training steps.}
%   \label{fig:primitivedistribution}
% \vspace{-0.3cm}
% \end{wrapfigure}
%\subsection{Complexity of the Environments}
\label{sec:complexity}
% \textbf{Environment complexity:} While agent performance improves over time, we would like to know if they are presented with more challenging environments over training.
% We estimate the number of active and passive primitives generated as a measure of environment complexity.
% Learning a web page with more passive primitives is a relatively easier task than a page with more active primitives, because passive primitives either add noise and should ignored by the agents, or are used by agents only to navigate to another page.
% On the other hand, if there are more active primitives, not only will the size of the DOM tree increase but the number of profile fields will increase, making the matching between elements and profile more challenging.
% %Figure \ref{fig:primitivedistribution} outlines the percentage of active primitives over time.
% \WEDPb\ starts around 60\% random selection of primitives, and gradually generates more active primitives early on (Figure \ref{fig:primitivedistribution}).
% Although presented with more active primitives by \WEDPb, agents are still able to improve thanks to \WEDPb's ability to accurately tune the difficulty of the environments according to agents' skill. During training, more and more passive primitives are also introduced where number of active primitives also keeps increasing (see Appendix \ref{ap:primitive_frequencies}). We also observe that the distribution of the primitives shifts later in the training to more complex and relevant primitives (see Appendix \ref{ap:primitives}). 
%Perhaps surprisingly, \WEDP\ is unable to offer a better curriculum and it doesn't go beyond random sampling of primitives.


\textbf{Environment complexity:} \WEDPb\ produces a curriculum of emerging complexity, estimated by the number of active and passive primitives. \WEDPb\ starts around 60\% random selection of primitives, and gradually generates more primitives while improving agent's  performance (Figure \ref{fig:primitivedistribution}). Over the course of training, both number of active and passive primitives increases (Appendix \ref{ap:primitive_frequencies}), and the distribution of the primitives shifts to more complex and relevant primitives later on (Appendix \ref{ap:primitives}). 
Learning a web page with more passive primitives is a relatively easier task than a page with more active primitives, because passive primitives either add noise and should ignored by the agents, or are used by agents only to navigate to another page.
In addition, active primitives, not only increase DOM tree size, but the number of profile fields as well, making the matching between elements and profile more challenging.
%Figure \ref{fig:primitivedistribution} outlines the percentage of active primitives over time.
%\WEDPb\ starts around 60\% random selection of primitives, and gradually generates more active primitives early on (Figure \ref{fig:primitivedistribution}).
\WEDPb\ agents continue to improve performance thanks to \WEDPb's ability to accurately tune the difficulty of the environments to agents' proficiency. 



% Aggregated results (over difficulty levels) for DR, CL, PopRegret, CoDE:
% Task name=login_pages
% Difficulty=0
% DR 0.0
% CL 0.11
% PopRegret 0.2
% CoDE 1.0
% -----------------------
% Difficulty=1
% DR 0.0
% CL 0.0
% PopRegret 0.2
% CoDE 1.0
% -----------------------
% Difficulty=2
% DR 0.0
% CL 0.0
% PopRegret 0.175
% CoDE 0.86499995
% -----------------------
% Difficulty=3
% DR 0.0
% CL 0.0
% PopRegret 0.144
% CoDE 0.91999996
% -----------------------
% Task name=address_pages
% Difficulty=0
% DR 0.0
% CL 0.0
% PopRegret 0.1
% CoDE 1.0
% -----------------------
% Difficulty=1
% DR 0.0
% CL 0.0
% PopRegret 0.06666667
% CoDE 1.0
% -----------------------
% Difficulty=2
% DR 0.0
% CL 0.0
% PopRegret 0.08
% CoDE 0.95600003
% -----------------------
% Difficulty=3
% DR 0.0
% CL 0.0
% PopRegret 0.085714296
% CoDE 0.96000004
% -----------------------
% Task name=shopping
% Difficulty=0
% DR 0.0
% CL 0.0
% PopRegret 0.1
% CoDE 0.95
% -----------------------
% Difficulty=1
% DR 0.0
% CL 0.0
% PopRegret 0.06666667
% CoDE 1.0
% -----------------------
% Difficulty=2
% DR 0.0
% CL 0.0
% PopRegret 0.044444446
% CoDE 0.9133333
% -----------------------
% Difficulty=3
% DR 0.0
% CL 0.0
% PopRegret 0.033333335
% CoDE 0.9333334
% -----------------------
% Task name=payment
% Difficulty=0
% DR 0.0
% CL 0.0
% PopRegret 0.18
% CoDE 0.87
% -----------------------
% Difficulty=1
% DR 0.0
% CL 0.0
% PopRegret 0.18
% CoDE 0.90666664
% -----------------------
% Difficulty=2
% DR 0.0
% CL 0.0
% PopRegret 0.120000005
% CoDE 0.975
% -----------------------
% Difficulty=3
% DR 0.0
% CL 0.0
% PopRegret 0.144
% CoDE 0.96400005
% -----------------------
% Task name=flight
% Difficulty=0
% DR 0.0
% CL 0.0
% PopRegret 0.27000004
% CoDE 1.0
% -----------------------
% Difficulty=1
% DR 0.0
% CL 0.0
% PopRegret 0.18499999
% CoDE 1.0
% -----------------------
% Difficulty=2
% DR 0.0
% CL 0.0
% PopRegret 0.18666665
% CoDE 0.9633333
% -----------------------
% Difficulty=3
% DR 0.0
% CL 0.0
% PopRegret 0.17714287
% CoDE 0.83428574
% -----------------------

==> src/model.tex <==


% \begin{figure}
% \centering
% \begin{tabular}{ccc}
%     \subfloat[A \textbf{fully specified} DOM primitive where a label is created and its text is assigned.]{
%       \includegraphics[width=0.2\linewidth]{img/Underspecified DOM-2-0.pdf}\label{fig:underspecified0}} & %\hspace{10pt}%
%     \subfloat[An \textbf{underspecified} DOM tree template. While text box is always included, its text and label element are variables.]
%{\includegraphics[width=0.2\linewidth]{img/Underspecified DOM-2-1.pdf}\label{fig:underspecified1}}& %\hspace{10pt}%
%     \subfloat[A \textbf{fully specified} DOM primitive where only the inner text within the text box is assigned.]{
%       \includegraphics[width=0.2\linewidth]{img/Underspecified DOM-2-2.pdf}\label{fig:underspecified2}}%\hspace{10pt}%
%     \end{tabular}
%     \caption{An example underspecified DOM tree template (b) and its instantiations (a,c) with different values. (*) indicates a variable; either an element or one of its attributes. (a) is used in Page 1 and (c) is used in Page 2 in Figure \ref{fig:rollout}.}
%     \label{fig:underspecified}
% \end{figure}


% \begin{figure}[t]
% \centering
% %\captionsetup[subfigure]{width=.8\imagewidth}%
% \begin{subfigure}{.3\linewidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{img/Underspecified DOM-2-0.pdf}
%   \caption{A \textbf{fully specified} DOM primitive where a label is created and its text is assigned.}
%   \label{fig:underspecified0}
% \end{subfigure}\hfil%
% \begin{subfigure}{.36\linewidth}
%   \centering
%   \includegraphics[width=.7\linewidth]{img/Underspecified DOM-2-1.pdf}
%   \caption{An \textbf{underspecified} DOM tree template. The text box is always included, its text and label element are variables.}
%   \label{fig:underspecified1}
% \end{subfigure}\hfil%
% \begin{subfigure}{.28\linewidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{img/Underspecified DOM-2-2.pdf}
%   \caption{A \textbf{fully specified} DOM primitive where only the inner text within the text box is assigned.}
%   \label{fig:underspecified2}
% \end{subfigure}
% \caption{\small An example underspecified DOM tree template (b) and its instantiations (a,c) with different values. (*) indicates a variable; either an element or one of its attributes. (a) is used in Page 1 and (c) is used in Page 2 in Figure \ref{fig:rollout}.}
% \label{fig:underspecified}
% \end{figure}

\begin{figure}[t]
\centering
%\vspace{-1.cm}
% \subfloat[]{
%   \includegraphics[width=0.3\linewidth]{img/Underspecified DOM-2-1.pdf}
%   \label{fig:underspecified1}
% }
%\hspace{0.25in}
\subfloat[]{
  \includegraphics[width=0.3\linewidth]{img/Underspecified DOM-2-0.pdf}
  \label{fig:underspecified0}
}
%\hspace{0.25in}
%\subfloat[\textbf{fully specified} primitive where only the inner text within the text box is assigned.]{
 \subfloat[]{
  \includegraphics[width=0.3\linewidth]{img/Underspecified DOM-2-2.pdf}
  \label{fig:underspecified2}
}
\caption{Two example DOM primitives that are used in Page 1 and Page 2 in Figure \ref{fig:rollout}. Each primitive is implemented in HTML that is parsed into a DOM tree.}
\label{fig:underspecified}
% \vspace*{-0.25in}
\end{figure}

%\vspace*{-0.1in}
\section{Learning to Design Environments}
%\vspace*{-0.1in}
This Section presents the generative MiniWob environment (Section \ref{sec:gmniniwob}), the \adversary\ neural network architecture (Section \ref{sec:adversary}) and the adversary training (Section \ref{sec:adversary_training}). 

\subsection{Generative MiniWoB (gMiniWoB) Environment}
\label{sec:gmniniwob}
%\subsection{Website Design}
Generative MiniWoB (gMiniWoB) is a framework to create environments for form-filling tasks as an implementation of the Petri Nets formalism described in Section \ref{sec:definition}.
We denote a \textit{website} as a hierarchical CPN where each webpage is represented as a page CPN, connected in a linked-list of gates to create the website.
Each page CPN is composed of a set of parallel form-filling primitives with an output place connecting to the transition that link to the next page (Figure \ref{fig:petris}).
To create a new environment $\mathcal{E}_w$, gMiniWoB starts with an empty website and gradually populates by adding primitives and transitions.
The order in which primitives are added defines how a webpage will be rendered as a state for the agent, facilitating controllable generation with a rich design set.

We represent a primitive as a DOM tree which is implemented in gMiniWoB using HTML (Figure \ref{fig:underspecified}).
Let's assume that we are given a list of DOM tree primitives $P$ and an empty web page $\mathcal{W}=(\mathcal{S}, \mathcal{C})$ where there is a single root node $\mathcal{S}$ and a list of primitives $\mathcal{C} \subset P$ which is initially empty.
By repetitively sampling new primitives from $P$ and appending them to $\mathcal{C}$, we create a new page, $\mathcal{W},$ which follows the order of primitives in $\mathcal{C}$ when rendered (see Figure \ref{fig:rollout}).
Transitions are implemented as events that are attached to elements in each page.
For example, a submit button opens a new page when clicked.

% Generative MiniWoB (gMiniWoB) creates website environments for form-filling tasks, which consist of a linked-list of webpages, $\mathcal{E}_w = [\mathcal{W}_1, \cdots, \mathcal{W}_{K}]$.
% Each webpage, $\mathcal{W}_i,$ is a DOM tree that contains a number of elements, such as fill-in boxes, drop downs, and buttons. 
% To create a new environment $\mathcal{E}_w,$ gMiniWoB starts with an empty website that is gradually populated by new pages, $\mathcal{W}_i$.
% A subset of elements are also augmented with events that enable page transitions.
% %The pages $\mathcal{W}_i$ are DOM trees and the links between two pages are implicitly defined by events attached to certain elements.
% For example, an "on-click" event on a Submit button on a page $\mathcal{W}_i,$ will link to a page $\mathcal{W}_{i+1}.$ 

% We formulate the website design as combining a set of \textit{primitive DOM sub-trees} that are general enough to create complex websites but also facilitate controllable generation.
% The order in which the primitives are combined also defines how the web page will be rendered as well.
% Let's assume that we are given a list of DOM tree primitives $\mathcal{T}$ and an empty web page $\mathcal{W}=(\mathcal{S}, \mathcal{C})$ where $\mathcal{S}$ is a single root node of the DOM tree and $\mathcal{C}$ is an ordered list of subtrees rooted at $\mathcal{S}$ which is initially empty. By repetitively sampling new primitives from $\mathcal{T}$ and appending them to $\mathcal{C}$, we create a new page, $\mathcal{W},$ which follows the order of primitives in $\mathcal{C}$ when rendered (see Figure \ref{fig:rollout}).

% We first create a set of \textit{underspecified DOM tree templates}, a sub-tree with certain elements and attributes are replaced with variables.
% Assigning values to variables in a template fully specifies a DOM tree primitive that is placed in a subtree $\mathcal{C}$ to create a new web page, $\mathcal{W}$ (Algorithm \ref{alg:primitive-generation}).
% For example, an input template (Figure \ref{fig:underspecified1}) as a variable label and text box with a common parent. There two ways to assign values, either by picking the label element and assigning a value to its text attribute (Figure \ref{fig:underspecified0}), assigning a value to the inner text of the text box and ignoring the label element (Figure \ref{fig:underspecified2}).



%%While the most general approach to designing DOM trees would be combining a set of arbitrary elements in a bottom-up approach, this would generate a large number of malformed websites that are semantically incoherent.
%%Consider the second page in Figure \ref{fig:rollout} where there is a text box and a label on the top that says ``First Name''.
%%Now, if we have had inserted the label on top of the `Username' text box in the first page, the website would become malformed as it is ambiguous if the text box refers to `username' or `first name'.


%%As a result, we formulate the website design as combining a set of \textit{primitive DOM sub-trees} that are general enough to create complex websites but can be combined safely in a tree structure.
%%We first create a set of \textit{underspecified DOM tree templates} where certain elements and attributes are replaced with variables.
%%By assigning values to variables in a template, a fully specified DOM tree primitive is generated that can be combined with other primitives to create a new web page.
%%The order in which the primitives are combined also defines how the web page will be rendered as well.
% Let's assume that we are given a list of DOM tree primitives $\mathcal{T}$ and an empty web page $\mathcal{W}=(\mathcal{S}, \mathcal{E})$ where $S$ is a single root node of the DOM tree and $E$ is an ordered list of subtrees rooted at $S$ which is initially empty.
% By repetitively sampling new primitives from $\mathcal{T}$ and appending them to $\mathcal{E}$, we create a new page which follows the order of primitives in $\mathcal{E}$ when rendered (see sample pages in Figure \ref{fig:rollout}).

\begin{figure}
 %   \vspace{-0.1in}
    \centering
    \includegraphics[scale=0.6]{img/Adversary_rollout_and_DOM.pdf}
    \caption{\small A sample rollout of the adversary for compositional environment generation for web navigation problem. An initial observation (Obs) is given at the beginning of the rollout. $f_0$, $f_K$, $f_L$, $f_P$, and $f_I$ denote networks for encoding initial observation, generating number of pages, page indices,\protect\footnotemark primitives, and encoding LSTM inputs, respectively.}
    \label{fig:rollout}
 %   \vspace{-0.5cm}
\end{figure}

\footnotetext {For simplicity of illustration, we show an example generation process where primitives are generated in an increasing order of the page indices; however, in our formulation (see Section~\ref{sec:adversary} for details), the page indices corresponding to consecutive LSTM timesteps do not necessarily increase monotonically.}

\paragraph{Design Primitives:} gMiniWoB implements 40 different design primitives, widely used across the web and include `navigation bars', `product carousels', `item decks', `web forms', `item carts', `dropdowns', etc.
Every primitive includes at least one actionable element (transition) that changes the DOM structure when the agent interacts with it.
% Each primitive belongs to one of the two categories based on their use in the reward computation: (i) \textbf{Active primitives (used)}, and (ii) \textbf{Passive primitives (not used)}.
% Both primitives are further divided into 2 categories.
% Some passive primitives are needed for navigation (such as a 'Login' button), while some others are not needed for navigation but only for generalization to real websites.
% Active primitives can be self-sufficient where actionable elements don't need to condition on other elements (such as 'Username' text box in Figure \ref{fig:underspecified0}), or can be dependent where actionable elements need others to fully understand their semantics (such as 'First Name' text box in Figure \ref{fig:underspecified2} where without the label, the text box is ambiguous).
$26$ of the $40$ primitives are active, while the rest are passive.
When an active primitive is added to a web page, the instruction automatically grows as well.
For example, adding `First Name' text box in Figure \ref{fig:underspecified2} also adds a new \textit{``firstname''} field into user instruction.
Expanding the instruction set makes active primitives more complicated to learn, while the passive primitives mostly serve as noise. However, real websites contain many distracting elements (passive primitives), so it is important for agents to learn to ignore them. Appendix \ref{ap:design_primitives} details all the design primitives used, and Appendix \ref{ap:test} shows the websites in the test set.
% Active primitives can also be categorized into 2 according to 


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.6]{img/Adversary rollout and DOM.pdf}
%     \caption{\small A sample rollout of the adversary for compositional environment generation for web navigation problem. An initial observation (Obs) is given at the beginning of the rollout. $f_0$, $f_K$, $f_L$, $f_P$, and $f_I$ denote networks for encoding initial observation, generating number of pages, page indices,\protect footnotemark primitives, and encoding LSTM inputs, respectively.\footnotetext {For simplicity of illustration, we show an example generation process where primitives are generated in an increasing order of the page indices; however, in our formulation (see Section~\ref{sec:adversary} for details), the page indices corresponding to consecutive LSTM timesteps do not necessarily increase monotonically.}}
%     \label{fig:rollout}
%     \vspace{-0.4cm}
% \end{figure}


\subsection{\Adversary\ Environment Decoder Architecture}
\label{sec:adversary}
We present a \adversary\ decoder policy for the compositional environment generation problem where the goal is to place a set of design primitives to a set of locations. \Adversary\ generates an environment, $\mathcal{E}_w = [\mathcal{W}_1, \cdots, \mathcal{W}_{K}].$ We assume fixed maximum number of pages $K$, although to control complexity, we allow pages and subtrees to be empty. 

We parametrize the adversary with a policy $\pi_E(a^A | o^A)$ s.t. 
%We model the adversary as an autoregressive bandit with a policy $\pi_A(a^A | o^A;\Theta_A)$ such that
\begin{equation}
    %\pi_E(a^A | o^A) &= \pi(k | K)\prod_{i=0}^N{\pi(a_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k) \pi(b_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k)}
    \pi_E(a^A | o^A) = \pi_{\mathcal{E}_w}(k | K)\prod_{i=0}^N{\pi(a_i, b_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k)}
\end{equation}
where $N$ is an upper limit on the number of outputs and maximum design budget (total number of primitives in the environment $\mathcal{E}_w$), $K$ is an upper limit on the number of pages, $a_i$ is a primitive. We augment the primitives described in Section \ref{sec:gmniniwob} with a special \texttt{SKIP} primitive that does nothing when executed by the renderer, to allow the \adversary\ to control the number of primitives added.
$b_i$ is a page index of where the primitive $a_i$ should be placed in on the page. Observation $o^A$ is an initial observation.
The \adversary\ first samples the number of locations $k$ from a parametrized Categorical distribution $Cat(0, K)$.
Conditioned on $o^A$, it executes an autoregressive model to generate a set of primitives and their corresponding locations within $[0,\cdots,k]$. $a^A$ is the resulting environment totalling at most $N$ primitives placed over $k$ pages.

The initial observation $o^A$ is sampled from the standard normal distribution, to allow the \adversary\ to diversify its design distribution.
This observation is encoded with a feed forward network $h_0=f_0(o^A)$ and $h_0$ is passed to another network $f_K$ that outputs a distribution over number of empty pages.
The same hidden state $h_0$ is passed to an LSTM network as the initial input vector. The LSTM output is used by two independent networks $f_P$ and $f_L$ to learn a distribution over design primitives and locations, respectively.
We sample an action (a primitive and its location) and encode by another network $f_I$ into a hidden state which is used as the input to the LSTM at the next step.
After $N$ steps, sampled design is sent to a renderer module to generate the environment (Figure \ref{fig:rollout}). 

The \adversary\ is domain independent, and creates a generic compositional task with $K$ linked sub tasks, each sub task sampled from the design primitives described in Section \ref{sec:definition}. Since the renderer interprets the design decisions and builds the environments for the \webnav\ agents to use, the \adversary\ architecture is domain agnostic.     

%%For the web navigation problem, $K$ denotes the number of pages in the website, locations ($b_i$) denote pages, and primitives ($a_i$) denote DOM tree primitives.
%%We illustrate a sample rollout of the adversary for web environment generation in Figure \ref{fig:rollout}.
%We augment the primitive design actions described in Section \ref{sec:gmniniwob} with a special \texttt{SKIP} action that does nothing when executed by the renderer. This allows the adversary to control the number of primitives added.

% We note that our model is not constrained to bandits and alternative models can easily be incorporated.
% By using bandits, we avoid costly rendering of partial websites after each design decision and LSTM's internal memory .

% If a web page is not accessible from any other page, we add a dummy element to the preceding page and attach an event that enables the transition.

\subsection{\Adversary\ Training}
\label{sec:adversary_training}
We train both the \adversary\ and \webnav\ agents with RL. 
At every training step $t,$ the \adversary\ generates an environment $\mathcal{E}_w(t).$ The \webnav\ training initializes population of agents $\mathcal{A} =\{A_i, i=1,\cdots,n_a\}$. The agents $A_i \in \mathcal{A}$ collect $M$ trajectories $\tau_{i,j}$ with returns $R_{i,j}$. $R_{i,j}$ is a discounted cumulative reward that agent $A_i$ observers by navigating the environment, $\mathcal{E}_w,$ and resulting in trajectory $\tau_{i,j} \sim \pi_{A_i}.$ 
The \webnav\ agents use the standard task related reward described in Section \ref{sec:definition} for training and out-of-box A2C with entropy \citep{a2c}. To train the \adversary, we present a new loss function which augments A2C with entropy with a custom loss function that encourages the adversary to control the complexity of the environment %, by presenting "just-the-right" challenge for the agents in $\mathcal{A}$
(Algorithm \ref{alg:bflexible}).

\SetKwComment{Comment}{~~$\triangleright$\ }{}
\SetCommentSty{itshape\color{black!60}}
\begin{algorithm}[tb]
% \SetAlgoLined
%\begin{algorithmic}[1]
 \textbf{Input: }{$\mathcal{A}$: Initialize the agents independently} \\
 \For {all training iterations}{
 $\mathcal{E}_w$ $\longleftarrow$ \adversary\ $\pi_E$ generates new environment \\
 \For {$i=1,\cdots,n_a$}{
 $R_{i} \longleftarrow 0$ \\
 \For {$j=1,\cdots,M$}{~
 $R_{i,j}$ $\longleftarrow$ Collect rewards for $A_i$ in the env. $\mathcal{E}_w$\\
 $R_{i} \longleftarrow R_{i} + \frac{R_{i,j}}{M}$ \Comment{Exp. return for $\mathcal{A}_i.$} \\
 }%\EndFor
 }%\EndFor
 $R^{A} \longleftarrow \max_i R_{i}$, $R^{P} \longleftarrow \E[R_{i}]$  \Comment{Maximum and mean expected return from the agents.} \\
 REGRET$(\mathcal{A}| \mathcal{E}_w) \longleftarrow R^{A} - R^{P}$ \Comment {Per \Eqref{eq:flexible_regret}.} \\
 Update \adversary\ per \Eqref{eq:loss} and REGRET$(\mathcal{A}| \mathcal{E}_w)$ as the reward. \Comment{Train \adversary\ .} \\
 Update parameters of $\forall A_i \in \mathcal{A}$ using $R_{i}$ returns in A2C. \Comment{Train \webnav\ agents.}
 }%\EndFor
%\end{algorithmic}
 \caption{b-Flexible PAIRED training. Joint training of the \adversary\ and \webnav\ agents.}
 \label{alg:bflexible}
\end{algorithm}

%-------------------------------BACKUP------------------------------
\iffalse
\begin{algorithm}[tb]
% \SetAlgoLined
\begin{algorithmic}[1]
 \State \textbf{Input:}{$\mathcal{A}$: Initialize the agents independently}
 \For {all training iterations}
 \State $\mathcal{E}_w$ $\longleftarrow$ Run the \adversary\ $\pi_E$ to generate a new environment
 \For {$i=1,\cdots,n_a$}
 \State $R_{i} \longleftarrow 0$
 \For {$j=1,\cdots,M$}
 \State $R_{i,j}$ $\longleftarrow$ Run agent $A_i \in \mathcal{A}$ in the env. $\mathcal{E}_w$ and collect rewards.
 \State $R_{i} \longleftarrow R_{i} + \frac{R_{i,j}}{M}$ \Comment{Expected return for agent $\mathcal{A}_i.$}
 \EndFor
 \EndFor
 \State $R^{A} \longleftarrow \max_i R_{i}$, $R^{P} \longleftarrow \E[R_{i}]$  \Comment{Maximum and mean expected return from the agents.}
 \State REGRET$(\mathcal{A}| \mathcal{E}_w) \longleftarrow R^{A} - R^{P}$ \Comment {Compute regret as in \Eqref{eq:flexible_regret}.}
 \State Update adversary using \Eqref{eq:loss} and REGRET$(\mathcal{A}| \mathcal{E}_w)$ as the reward. \Comment{Train adversary.}
 \State Update parameters of $\forall A_i \in \mathcal{A}$ using $R_{i}$ returns in A2C. \Comment{Train navigation agents.} 
 \EndFor
\end{algorithmic}
 \caption{b-Flexible PAIRED training. Joint training of the adversary and navigation agents.}
 \label{alg:bflexible}
\end{algorithm}
\fi
%-----------

\subsubsection{Loss functions}
\label{sec:loss_functions}
Let $R_{i,j}(t)$ be observed returns (cumulative discounted reward) of an agent $A_i(t) \in \mathcal{A}$ while sampling $j^{\text{th}}$ trajectory during training iteration $t.$ Let $R^A$ and $R^P$ be maximum and average expected returns at the iteration $t$,
\begin{align}
    R^A &= \max_i \E(R_i), \; R^P =\E[\E[R_i]],\\
    \E[R_i] &= \frac{1}{M} \sum_{j} R_{i,j},\, i=1,\cdots,M \label{eq:a_p}
\end{align}
Then, the \adversary\ loss function consists of two terms,
\begin{multline}
    \mathcal{J}(\theta|\mathcal{A}, \mathcal{E}_w) = (1-\alpha) * \mathcal{J}_{\text{rl}}(\theta\,|\,\textsc{REGRET}(\mathcal{A}|\mathcal{E}_w)) \\
     + \alpha * \mathcal{J}_{\text{budget}}(\theta\,|\,\mathcal{A}, \mathcal{E}_w)
    \label{eq:loss} 
\end{multline}
where $\alpha$ is a balancing factor between the two losses.
$\mathcal{J}_{\text{rl}}$ is standard A2C loss with cross-entropy regularizer added to encourage adversary's exploration. The reward function for the $\mathcal{J}_{\text{rl}}$ is regret, estimated as the difference between expected performance of the best and average agents:  
\begin{equation}
    \textsc{REGRET}(\mathcal{A}|\mathcal{E}_w) = R^A - R^P. \label{eq:flexible_regret}
\end{equation}
The second loss term $\mathcal{J}_{\text{budget}}(\theta\,|\,\mathcal{A}, \mathcal{E}_w)$ is the budget loss,
\begin{equation}
    R^A * \sum_{i=1}^N{\log  \pi_{\theta}(a_i=\text{SKIP}|a_{0\cdots i-1}, b_{0 \cdots i-1})}. \label{eq:budget}
\end{equation}
We use an environment difficulty objective to bind the \adversary's design budget to the performance of the best agent. We approximate the effective budget of the \adversary\ as the expected number of non-SKIP actions over $N$ time steps and update this budget according to whether the agents are learning. This objective encourages the \adversary\ to use less budget (more SKIP actions) when the agents are not yet learning (i.e.,  $R^A$ is negative or low); it encourages the \adversary\ to use more budget (less SKIP actions) when the \webnav\ agents are performing well and collecting positive rewards in the environment. On the flip side, when the agents are collecting negative reward, the \adversary\ is encouraged to decrease the budget and sample less design elements (and more SKIP actions).

\subsubsection{Loss functions discussion}
Budget loss provides training signal for the \adversary\ when the regret reward is sparse, which happens when all agents are performing very similarly, and it acts to encourage the \adversary\ to decrease the difficulty of the environment.
Consider the scenario where agents are placed on the home page of a shopping website where there are many possible elements, but only a single button that takes them to their account page. During exploration, agents mostly collect negative rewards for taking incorrect actions, bounded to a very narrow interval (as there is only a single optimal action).
In this case, the regret is very small and sparse, which hinders the \adversary's ability to design environments at an appropriate difficulty for agents to learn.
We approximate the environment difficulty and the effective budget of the \adversary\ as a monotonic function of number of non-SKIP actions over $N$ created elements, and update this budget according to whether the agents are learning.
% This objective encourages the adversary to generate easier environments by using less budget (more SKIP actions) when the agents are not yet learning (i.e.,  $R^A$ is negative or low); it encourages the adversary to create difficult environments and use more budget (less SKIP actions) when the \webnav\ agents are collecting positive rewards in the environment.

The regret presented in \Eqref{eq:flexible_regret} contributes two subtle, but important changes over the prior work. First, the presented regret does not make a distinction between antagonist and protagonist agents, and instead annotates the best performing agent as the antagonist.
As long as any agent has a higher performance than the other agent, the objective will continue to improve the weakest agent.
During that time, the other agents continue learning, and therefore provide a stronger maximum performance against which we measure the regret. We call this objective as \WEDPb.
Second, the estimates for the protagonist are smoothed and computed as a best mean return, instead of maximum of a pre-selected agent. While this might be further underestimating the regret, it provides a more stable estimate.

Note that when the \adversary\ creates non-trivial environments, REGRET is close to zero and the budget loss in \Eqref{eq:budget} dominates the RL loss. However, when the \adversary\ creates trivial websites, the RL loss and regret encourage the \adversary\ to explore towards environments that promote variation in performance. Those are less trivial, hence it pushes the \adversary\ towards increasing the difficulty.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Website Design}
% We start with an empty website that is gradually populated by new pages and links between them.
% Given that we represent pages by their DOM, we focus on creating DOM trees and assume links between pages are implicitly defined by events attached to certain elements.


% While the most general approach to designing DOM trees would be combining a set of arbitrary elements in a bottom-up approach, this would generate a large number of malformed websites that are semantically incoherent.
% Consider the second page in Figure \ref{fig:rollout} where there is a text box and a label on the top that says ``First Name''.
% Now, if we have had inserted the label on top of the `Username' text box in the first page, the website would become malformed as it is ambiguous if the text box refers to `username' or `first name'.


% As a result, we formulate the website design as combining a set of \textit{primitive DOM sub-trees} that are general enough to create complex websites but can be combined safely in a tree structure.
% We first create a set of \textit{underspecified DOM tree templates} where certain elements and attributes are replaced with variables.
% By assigning values to variables in a template, a fully specified DOM tree primitive is generated that can be combined with other primitives to create a new web page.
% The order in which the primitives are combined also defines how the web page will be rendered as well.
% % Let's assume that we are given a list of DOM tree primitives $\mathcal{T}$ and an empty web page $\mathcal{W}=(\mathcal{S}, \mathcal{E})$ where $S$ is a single root node of the DOM tree and $E$ is an ordered list of subtrees rooted at $S$ which is initially empty.
% % By repetitively sampling new primitives from $\mathcal{T}$ and appending them to $\mathcal{E}$, we create a new page which follows the order of primitives in $\mathcal{E}$ when rendered (see sample pages in Figure \ref{fig:rollout}).


% Figure \ref{fig:underspecified} illustrates an example underspecified DOM tree template and its instantiations with different variable assignments.
% We create an input template (Figure \ref{fig:underspecified1}) as a variable label and text box with a common parent.
% In Figure \ref{fig:underspecified0}, we pick the label element and assign a value to its text attribute while in Figure \ref{fig:underspecified2}, we assign a value to the inner text of the text box and ignore the label element.


% \subsection{Website Design Primitives}
% We introduce a new framework called gMiniWoB for automated website generation, 
% which implements 40 different design primitives from 11 different underspecified DOM templates.
% These primitives are widely used across the web and include `navigation bars', `product carousels', `item decks', `web forms', `item carts', `dropdowns', etc.
% Every primitive includes at least one actionable element that changes the DOM structure when the agent interacts with it.
% Each primitive is classified into 2 different categories based on their use in the reward computation: (i) \textbf{Active primitives (used)}, and (ii) \textbf{Passive primitives (not used)}.
% % Both primitives are further divided into 2 categories.
% % Some passive primitives are needed for navigation (such as a 'Login' button), while some others are not needed for navigation but only for generalization to real websites.
% % Active primitives can be self-sufficient where actionable elements don't need to condition on other elements (such as 'Username' text box in Figure \ref{fig:underspecified0}), or can be dependent where actionable elements need others to fully understand their semantics (such as 'First Name' text box in Figure \ref{fig:underspecified2} where without the label, the text box is ambiguous).
% $26$ of the $40$ different primitives are active primitives and the rest are passive.
% When a new active primitive is added to a web page, it automatically also grows the instruction to accommodate the corresponding field.
% For example, adding `First Name' text box in Figure \ref{fig:underspecified2} also adds a new field with \textit{``firstname''} key into user instruction.
% This makes active primitives more complicated to learn than passive primitives, which mostly serve as noise. However, real websites contain many distracting elements (passive primitives), so it is important for agents to learn to ignore them. Appendix \ref{ap:design_primitives} details all the design primitives used, and Appendix \ref{ap:test} shows the websites in the testset.
% % Active primitives can also be categorized into 2 according to 

% \subsection{Adversary Architecture}
% \label{sec:adversary}
% % Given a list of design primitives, the goal of the adversary is to create a set of empty pages in the website and assign a subset of these primitives to pages.
% We propose an autoregressive adversary policy for the compositional environment generation problem where the goal is to place a set of design primitives to a set of locations.
% We parametrize the adversary with a policy $\pi_E(a^A | o^A)$ such that 
% %We model the adversary as an autoregressive bandit with a policy $\pi_A(a^A | o^A;\Theta_A)$ such that
% \begin{align}
%     \pi_E(a^A | o^A) &= \pi(k | K)\prod_{i=0}^N{\pi(a_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k) \pi(b_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k)}
% \end{align}
% where $N$ is an upper limit on the number of outputs, $K$ is an upper limit on the number of locations, $a_i$ is a design primitive, $b_i$ is a location index, and $o^A$ is an initial observation.
% The adversary first samples the number of locations $k$ from a parametrized Categorical distribution $Cat(0, K)$.
% Conditioned on $o^A$, it executes an autoregressive model to generate a set of primitives and their corresponding locations within $[0,\cdots,k]$.

% We sample $o^A$ from the standard normal distribution, similar to generative adversarial networks (GAN), to allow the adversary to diversify its design distribution.
% This observation is encoded with a feed forward network $h_0=f_0(o^A)$ and $h_0$ is passed to another network $f_K$ that outputs a distribution over number of empty pages.
% The same hidden state $h_0$ is passed to an LSTM network as the initial input vector and output of the LSTM is used by two independent networks $f_P$ and $f_L$ to (i) learn a distribution over design primitives and (ii) learn a distribution over locations, respectively.
% We sample a primitive and a location from these distributions and they are encoded by another network $f_I$ into a hidden state which is used as the input to the LSTM at the next step.
% After running for $N$ steps, sampled design actions are sent to a renderer module which generates the environment.

% For the web navigation problem, $K$ denotes the number of pages in the website, locations ($b_i$) denote pages, and primitives ($a_i$) denote DOM tree primitives.
% We illustrate a sample rollout of the adversary for web environment generation in Figure \ref{fig:rollout}.
% We also augment the primitive design actions with a special \texttt{SKIP} action that does nothing when executed by the renderer.
% This allows the adversary to control the number of primitives added.

% We note that our model is not constrained to bandits and alternative models can easily be incorporated.
% By using bandits, we avoid costly rendering of partial websites after each design decision and LSTM's internal memory .

% If a web page is not accessible from any other page, we add a dummy element to the preceding page and attach an event that enables the transition.

% \subsection{Population-based regret computation}
% \label{sec:our_regret}
% We leverage population-based training (PBT) to improve on the regret objective of Eq. \ref{eq:paired_regret}.
% We initialize a population of agents $\mathcal{P}$. At each iteration, the adversary designs a new website and each agent collects a set of rewards by navigating the website. After taking the mean of these rewards, we compute the regret using the population as follows:
% \begin{equation}
%     \textsc{REGRET} = \max_{i \in \mathcal{P}}\mathbb{E}[R_i] - \mathbb{E}_{j \in \mathcal{P}}\mathbb{E}[R_j]
%     \label{eq:our_regret}
% \end{equation}
% This objective does not make a distinction between antagonist and protagonist agents, and instead combines them into a single population. As such, it does not suffer from the shortcoming of the PAIRED objective which was limited by the performance of a single antagonist. As long as any agent in the population has lower performance than any other agent, the objective will continue to improve the weakest agent. During that time, the other agents in the policy continue learning, and therefore provide a stronger maximum performance against which we measure the regret. If the system reaches an equilibrium, each agent will be playing the minimum regret policy with respect to the population. 

% The combined population algorithm we propose is shown below. Using policy gradient updates, we train each agent in the population to optimize environmental reward, and the adversary to maximize the regret as computed in Eq. \ref{eq:our_regret}.

% \begin{algorithm}[H]
% % \SetAlgoLined
% \begin{algorithmic}[1]
%  \State \textbf{Input:}{$P_A$: A population of antagonist agents}
%  \State \textbf{Input:} $P_P$: A population of protagonist agents
%  \State $W$ $\longleftarrow$ Run the adversary $\pi_A$ to generate a new website
%  \For{Each antagonist and protagonist agent $j \in P_A \cup P_P$}
%     \State Run agent $j$ in the environment $W$ for $m$ episodes and collect rewards $R_{j,m}$
%  \EndFor
%  \State REGRET $\longleftarrow max_{j \in P_A}(mean_m(R_{j,m})) - mean_{j \in P_P}(mean_m(R_{j,m}))$
%  \State Update adversary parameters using REGRET as the reward
%  \For{Each antagonist and protagonist agent $j \in P_A \cup P_P$}
%     \State Update agent parameters $j$ using its corresponding reward $R_{j,m}$
%  \EndFor
% \end{algorithmic}
%  \caption{One step training of adversary and population of agents}
% \end{algorithm}

% As an ablation, we also experiment with maintaining a separate population of antagonist and protagonist agents, to more closely approximate the original PAIRED objective. In this case, we compute $\textsc{REGRET} = \max_{i \in \mathcal{P}_A}\mathbb{E}[R_i] - \mathbb{E}_{j \in \mathcal{P}_P}\mathbb{E}[R_j]$, where $\mathcal{P}_A$ and $P_P$ are antagonist and protagonist agent populations, respectively. Our experiments show that our combined population approach gives superior performance to this objective. 

%\todo[inline]{Izzet: Below is an alternative to population training section if we decide to exclude it for now.}
%NJ: looks good
%\subsection{Flexible PAIRED}
%\label{sec:flexible}
% We use flexible antagonist selection to improve on the regret objective of Eq. \ref{eq:paired_regret}.
% We initialize two agents $A$ and $P$. At each iteration, the adversary designs a new website and each agent collects a trajectory with return $R$ by navigating the website and the regret is:
% \begin{equation}
%     \textsc{REGRET} = \max \{R^A, R^P\} - 0.5 * (R^A+R^P) \label{eq:flexible_regret}
% \end{equation}
% \begin{equation}
%     \textsc{REGRET} = \max \{R(\tau^A), R(\tau^P)\} - 0.5 * (R(\tau^A)+R(\tau^P)) \label{eq:flexible_regret}
% \end{equation}
% \begin{equation}
%     \textsc{REGRET} = \max_{\mathcal{A},\mathcal{P}} ({\mathbb{E}[R_\mathcal{A}], \mathbb{E}[R_\mathcal{P}]}) - \mathbb{E}_{\mathcal{A},\mathcal{P}}{[0.5 *(R_\mathcal{A}+R_\mathcal{P})]}
%     \label{eq:flexible_regret}
% \end{equation}
% This objective does not make a distinction between antagonist and protagonist agents, and instead annotates the best performing agent as the antagonist.
% As long as any agent has a higher performance than the other agent, the objective will continue to improve the weakest agent.
% During that time, the other agent in the policy continues learning, and therefore provide a stronger maximum performance against which we measure the regret. The Flexible PAIRED algorithm we propose is shown below. Using policy gradient updates, we train each agent in the population to optimize environmental reward, and the adversary to maximize the regret as computed in Eq. \ref{eq:flexible_regret}.

% \begin{algorithm}[H]
% % \SetAlgoLined
% \begin{algorithmic}[1]
%  \State \textbf{Input:}{$A,P$: Initialize two agents independently}
%  \State $W$ $\longleftarrow$ Run the adversary $\pi_E$ to generate a new website
%  \State $R_{A}$, $R_{P}$ $\longleftarrow$ Run agent $A$ and $\mathcal{P}$ in the environment $W$ for $M$ episodes and collect rewards
%  \State REGRET $\leftarrow \frac{1}{M} (\max_{\mathcal{A},\mathcal{P}} (\sum_{m=1}^M{R_{\mathcal{A}, m}}, \sum_{m=1}^M{R_{\mathcal{P}, m}}) - 0.5(\sum_{m=1}^M{R_{\mathcal{A}, m}} + \sum_{m=1}^M{R_{\mathcal{P}, m}}))$
%  \State Update adversary parameters using REGRET as the reward
%  \State Update parameters of $A$ and $\mathcal{P}$ using $R_{A,m}$ and $R_{\mathcal{P},m}$, respectively
% \end{algorithmic}
%  \caption{One step training of flexible PAIRED}
% \end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}[H]
% % \SetAlgoLined
% \begin{algorithmic}[1]
%  \State \textbf{Input:}{$A,P$: Initialize two agents independently}
%  \State $W$ $\longleftarrow$ Run the adversary $\pi_E$ to generate a new website
%  \State $R^{A}$, $R^{P}$ $\longleftarrow$ Run agent $A$ and $P$ in the environment $W$ and collect rewards
%  \State REGRET $\longleftarrow$ Compute regret as in Eq. \ref{eq:flexible_regret}
%  \State Update adversary parameters using REGRET as the reward
%  \State Update parameters of $A$ and $P$ using $R^{A}$ and $R^{P}$, respectively
% \end{algorithmic}
%  \caption{One step training of flexible PAIRED}
%  \label{alg:bflexible}
% \end{algorithm}

% \subsection{Budget Enforcing on Adversary}
% Consider the following scenario where agents are placed on the home page of a shopping website where there are many possible elements, but only a single button that takes them to their account page.
% During exploration, agents mostly collect negative rewards for taking incorrect actions, bounded to a very narrow interval (as there is only a single optimal action).
% In this case, the regret is very small and non-informative, which hinders the adversary's ability to design environments at an appropriate difficulty for agents to learn.
% This is true even with the proposed flexible regret objective.
% % Intuitively, adversary should increase/decrease environment's difficulty only if antagonist agents 

% To mitigate this problem, we use a budget enforcing objective in addition to the regret that binds the adversary's design budget to the performance of the best agent.
% We approximate the effective budget of the adversary as the expected number of non-SKIP actions over $N$ time steps and update this budget according to whether the agents are learning.
% More formally, we use the following minimization objective for budget enforcing that is added to the PAIRED objective:
% \begin{equation}
%     \mathcal{O}_{budget} = R^A * \sum_{i=1}^N{\log  \pi(a_i=\text{SKIP}|a_{0\cdots i-1}, b_{0,\cdots, i-1})}
%     \label{eq:loss}
% \end{equation}
% where $R^A$ is the reward of the antagonist (or the best-performing) agent.
% This objective encourages the adversary to use less budget (more SKIP actions) when the agents are not yet learning (i.e.,  $R^A$ is negative or low); it encourages the adversary to use more budget (less SKIP actions) when the \webnav\ agents are collecting positive rewards in the environment.


==> src/model_before_rebuttal.tex <==


% \begin{figure}
% \centering
% \begin{tabular}{ccc}
%     \subfloat[A \textbf{fully specified} DOM primitive where a label is created and its text is assigned.]{
%       \includegraphics[width=0.2\linewidth]{img/Underspecified DOM-2-0.pdf}\label{fig:underspecified0}} & %\hspace{10pt}%
%     \subfloat[An \textbf{underspecified} DOM tree template. While text box is always included, its text and label element are variables.]
%{\includegraphics[width=0.2\linewidth]{img/Underspecified DOM-2-1.pdf}\label{fig:underspecified1}}& %\hspace{10pt}%
%     \subfloat[A \textbf{fully specified} DOM primitive where only the inner text within the text box is assigned.]{
%       \includegraphics[width=0.2\linewidth]{img/Underspecified DOM-2-2.pdf}\label{fig:underspecified2}}%\hspace{10pt}%
%     \end{tabular}
%     \caption{An example underspecified DOM tree template (b) and its instantiations (a,c) with different values. (*) indicates a variable; either an element or one of its attributes. (a) is used in Page 1 and (c) is used in Page 2 in Figure \ref{fig:rollout}.}
%     \label{fig:underspecified}
% \end{figure}


% \begin{figure}[t]
% \centering
% %\captionsetup[subfigure]{width=.8\imagewidth}%
% \begin{subfigure}{.3\linewidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{img/Underspecified DOM-2-0.pdf}
%   \caption{A \textbf{fully specified} DOM primitive where a label is created and its text is assigned.}
%   \label{fig:underspecified0}
% \end{subfigure}\hfil%
% \begin{subfigure}{.36\linewidth}
%   \centering
%   \includegraphics[width=.7\linewidth]{img/Underspecified DOM-2-1.pdf}
%   \caption{An \textbf{underspecified} DOM tree template. The text box is always included, its text and label element are variables.}
%   \label{fig:underspecified1}
% \end{subfigure}\hfil%
% \begin{subfigure}{.28\linewidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{img/Underspecified DOM-2-2.pdf}
%   \caption{A \textbf{fully specified} DOM primitive where only the inner text within the text box is assigned.}
%   \label{fig:underspecified2}
% \end{subfigure}
% \caption{\small An example underspecified DOM tree template (b) and its instantiations (a,c) with different values. (*) indicates a variable; either an element or one of its attributes. (a) is used in Page 1 and (c) is used in Page 2 in Figure \ref{fig:rollout}.}
% \label{fig:underspecified}
% \end{figure}

\begin{figure}[t]
\centering
\vspace{-1.cm}
\subfloat[An \textbf{underspecified} DOM tree template. The text box is always included, its text and label element are variables.]{
  \includegraphics[width=0.28\linewidth]{img/Underspecified DOM-2-1.pdf}
  \label{fig:underspecified1}
}
\hspace{0.15in}
\subfloat[A \textbf{fully specified} DOM primitive where a label is created and its text is assigned.]{
  \includegraphics[width=0.28\linewidth]{img/Underspecified DOM-2-0.pdf}
  \label{fig:underspecified0}
}
\hspace{0.15in}
\subfloat[A \textbf{fully specified} DOM primitive where only the inner text within the text box is assigned.]{
  \includegraphics[width=0.28\linewidth]{img/Underspecified DOM-2-2.pdf}
  \label{fig:underspecified2}
}
\caption{An example underspecified DOM tree template (a) and its instantiations (b,c) with different values. (*) indicates a variable; either an element or one of its attributes. (a) is used in Page 1 and (c) is used in Page 2 in Figure \ref{fig:rollout}.}
\label{fig:underspecified}
\end{figure}

\section{Learning to Design Web Environments}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Website Design}
We start with an empty website that is gradually populated by new pages and links between them.
Given that we represent pages by their DOM, we focus on creating DOM trees and assume links between pages are implicitly defined by events attached to certain elements.


While the most general approach to designing DOM trees would be combining a set of arbitrary elements in a bottom-up approach, this would generate a large number of malformed websites that are semantically incoherent.
Consider the second page in Figure \ref{fig:rollout} where there is a text box and a label on the top that says ``First Name''.
Now, if we have had inserted the label on top of the `Username' text box in the first page, the website would become malformed as it is ambiguous if the text box refers to `username' or `first name'.


As a result, we formulate the website design as combining a set of \textit{primitive DOM sub-trees} that are general enough to create complex websites but can be combined safely in a tree structure.
We first create a set of \textit{underspecified DOM tree templates} where certain elements and attributes are replaced with variables.
By assigning values to variables in a template, a fully specified DOM tree primitive is generated that can be combined with other primitives to create a new web page.
The order in which the primitives are combined also defines how the web page will be rendered as well.
% Let's assume that we are given a list of DOM tree primitives $\mathcal{T}$ and an empty web page $\mathcal{W}=(\mathcal{S}, \mathcal{E})$ where $S$ is a single root node of the DOM tree and $E$ is an ordered list of subtrees rooted at $S$ which is initially empty.
% By repetitively sampling new primitives from $\mathcal{T}$ and appending them to $\mathcal{E}$, we create a new page which follows the order of primitives in $\mathcal{E}$ when rendered (see sample pages in Figure \ref{fig:rollout}).


Figure \ref{fig:underspecified} illustrates an example underspecified DOM tree template and its instantiations with different variable assignments.
We create an input template (Figure \ref{fig:underspecified1}) as a variable label and text box with a common parent.
In Figure \ref{fig:underspecified0}, we pick the label element and assign a value to its text attribute while in Figure \ref{fig:underspecified2}, we assign a value to the inner text of the text box and ignore the label element.

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{img/Adversary rollout and DOM.pdf}
    \caption{\small A sample rollout of the adversary for compositional environment generation for web navigation problem. An initial observation (Obs) is given at the beginning of the rollout. $f_0$, $f_K$, $f_L$, $f_P$, and $f_I$ denote networks for encoding initial observation, generating number of pages, page indices,\protect\footnotemark primitives, and encoding LSTM inputs, respectively.}
    \label{fig:rollout}
    \vspace{-0.4cm}
\end{figure}

\footnotetext {For simplicity of illustration, we show an example generation process where primitives are generated in an increasing order of the page indices; however, in our formulation (see Section~\ref{sec:adversary} for details), the page indices corresponding to consecutive LSTM timesteps do not necessarily increase monotonically.}

\subsection{Website Design Primitives}
We introduce a new framework called gMiniWoB for automated website generation, 
which implements 40 different design primitives from 11 different underspecified DOM templates.
These primitives are widely used across the web and include `navigation bars', `product carousels', `item decks', `web forms', `item carts', `dropdowns', etc.
Every primitive includes at least one actionable element that changes the DOM structure when the agent interacts with it.
Each primitive is classified into 2 different categories based on their use in the reward computation: (i) \textbf{Active primitives (used)}, and (ii) \textbf{Passive primitives (not used)}.
% Both primitives are further divided into 2 categories.
% Some passive primitives are needed for navigation (such as a 'Login' button), while some others are not needed for navigation but only for generalization to real websites.
% Active primitives can be self-sufficient where actionable elements don't need to condition on other elements (such as 'Username' text box in Figure \ref{fig:underspecified0}), or can be dependent where actionable elements need others to fully understand their semantics (such as 'First Name' text box in Figure \ref{fig:underspecified2} where without the label, the text box is ambiguous).
$26$ of the $40$ different primitives are active primitives and the rest are passive.
When a new active primitive is added to a web page, it automatically also grows the instruction to accommodate the corresponding field.
For example, adding `First Name' text box in Figure \ref{fig:underspecified2} also adds a new field with \textit{``firstname''} key into user instruction.
This makes active primitives more complicated to learn than passive primitives, which mostly serve as noise. However, real websites contain many distracting elements (passive primitives), so it is important for agents to learn to ignore them. Appendix \ref{ap:design_primitives} details all the design primitives used, and Appendix \ref{ap:test} shows the websites in the testset.
% Active primitives can also be categorized into 2 according to 

\subsection{Adversary Architecture}
\label{sec:adversary}
% Given a list of design primitives, the goal of the adversary is to create a set of empty pages in the website and assign a subset of these primitives to pages.
We propose an autoregressive adversary policy for the compositional environment generation problem where the goal is to place a set of design primitives to a set of locations.
We parametrize the adversary with a policy $\pi_E(a^A | o^A)$ such that 
%We model the adversary as an autoregressive bandit with a policy $\pi_A(a^A | o^A;\Theta_A)$ such that
\begin{align}
    \pi_E(a^A | o^A) &= \pi(k | K)\prod_{i=0}^N{\pi(a_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k) \pi(b_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k)}
\end{align}
where $N$ is an upper limit on the number of outputs, $K$ is an upper limit on the number of locations, $a_i$ is a design primitive, $b_i$ is a location index, and $o^A$ is an initial observation.
The adversary first samples the number of locations $k$ from a parametrized Categorical distribution $Cat(0, K)$.
Conditioned on $o^A$, it executes an autoregressive model to generate a set of primitives and their corresponding locations within $[0,\cdots,k]$.

We sample $o^A$ from the standard normal distribution, similar to generative adversarial networks (GAN), to allow the adversary to diversify its design distribution.
This observation is encoded with a feed forward network $h_0=f_0(o^A)$ and $h_0$ is passed to another network $f_K$ that outputs a distribution over number of empty pages.
The same hidden state $h_0$ is passed to an LSTM network as the initial input vector and output of the LSTM is used by two independent networks $f_P$ and $f_L$ to (i) learn a distribution over design primitives and (ii) learn a distribution over locations, respectively.
We sample a primitive and a location from these distributions and they are encoded by another network $f_I$ into a hidden state which is used as the input to the LSTM at the next step.
After running for $N$ steps, sampled design actions are sent to a renderer module which generates the environment.

For the web navigation problem, $K$ denotes the number of pages in the website, locations ($b_i$) denote pages, and primitives ($a_i$) denote DOM tree primitives.
We illustrate a sample rollout of the adversary for web environment generation in Figure \ref{fig:rollout}.
We also augment the primitive design actions with a special \texttt{SKIP} action that does nothing when executed by the renderer.
This allows the adversary to control the number of primitives added.

% We note that our model is not constrained to bandits and alternative models can easily be incorporated.
% By using bandits, we avoid costly rendering of partial websites after each design decision and LSTM's internal memory .

% If a web page is not accessible from any other page, we add a dummy element to the preceding page and attach an event that enables the transition.

% \subsection{Population-based regret computation}
% \label{sec:our_regret}
% We leverage population-based training (PBT) to improve on the regret objective of Eq. \ref{eq:paired_regret}.
% We initialize a population of agents $\mathcal{P}$. At each iteration, the adversary designs a new website and each agent collects a set of rewards by navigating the website. After taking the mean of these rewards, we compute the regret using the population as follows:
% \begin{equation}
%     \textsc{REGRET} = \max_{i \in \mathcal{P}}\mathbb{E}[R_i] - \mathbb{E}_{j \in \mathcal{P}}\mathbb{E}[R_j]
%     \label{eq:our_regret}
% \end{equation}
% This objective does not make a distinction between antagonist and protagonist agents, and instead combines them into a single population. As such, it does not suffer from the shortcoming of the PAIRED objective which was limited by the performance of a single antagonist. As long as any agent in the population has lower performance than any other agent, the objective will continue to improve the weakest agent. During that time, the other agents in the policy continue learning, and therefore provide a stronger maximum performance against which we measure the regret. If the system reaches an equilibrium, each agent will be playing the minimum regret policy with respect to the population. 

% The combined population algorithm we propose is shown below. Using policy gradient updates, we train each agent in the population to optimize environmental reward, and the adversary to maximize the regret as computed in Eq. \ref{eq:our_regret}.

% \begin{algorithm}[H]
% % \SetAlgoLined
% \begin{algorithmic}[1]
%  \State \textbf{Input:}{$P_A$: A population of antagonist agents}
%  \State \textbf{Input:} $P_P$: A population of protagonist agents
%  \State $W$ $\longleftarrow$ Run the adversary $\pi_A$ to generate a new website
%  \For{Each antagonist and protagonist agent $j \in P_A \cup P_P$}
%     \State Run agent $j$ in the environment $W$ for $m$ episodes and collect rewards $R_{j,m}$
%  \EndFor
%  \State REGRET $\longleftarrow max_{j \in P_A}(mean_m(R_{j,m})) - mean_{j \in P_P}(mean_m(R_{j,m}))$
%  \State Update adversary parameters using REGRET as the reward
%  \For{Each antagonist and protagonist agent $j \in P_A \cup P_P$}
%     \State Update agent parameters $j$ using its corresponding reward $R_{j,m}$
%  \EndFor
% \end{algorithmic}
%  \caption{One step training of adversary and population of agents}
% \end{algorithm}

% As an ablation, we also experiment with maintaining a separate population of antagonist and protagonist agents, to more closely approximate the original PAIRED objective. In this case, we compute $\textsc{REGRET} = \max_{i \in \mathcal{P}_A}\mathbb{E}[R_i] - \mathbb{E}_{j \in \mathcal{P}_P}\mathbb{E}[R_j]$, where $\mathcal{P}_A$ and $P_P$ are antagonist and protagonist agent populations, respectively. Our experiments show that our combined population approach gives superior performance to this objective. 

%\todo[inline]{Izzet: Below is an alternative to population training section if we decide to exclude it for now.}
%NJ: looks good
\subsection{Flexible PAIRED}
\label{sec:flexible}
We use flexible antagonist selection to improve on the regret objective of Eq. \ref{eq:paired_regret}.
We initialize two agents $A$ and $P$. At each iteration, the adversary designs a new website and each agent collects a trajectory with return $R$ by navigating the website and the regret is:
\begin{equation}
    \textsc{REGRET} = \max \{R^A, R^P\} - 0.5 * (R^A+R^P) \label{eq:flexible_regret}
\end{equation}
% \begin{equation}
%     \textsc{REGRET} = \max \{R(\tau^A), R(\tau^P)\} - 0.5 * (R(\tau^A)+R(\tau^P)) \label{eq:flexible_regret}
% \end{equation}
% \begin{equation}
%     \textsc{REGRET} = \max_{\mathcal{A},\mathcal{P}} ({\mathbb{E}[R_\mathcal{A}], \mathbb{E}[R_\mathcal{P}]}) - \mathbb{E}_{\mathcal{A},\mathcal{P}}{[0.5 *(R_\mathcal{A}+R_\mathcal{P})]}
%     \label{eq:flexible_regret}
% \end{equation}
This objective does not make a distinction between antagonist and protagonist agents, and instead annotates the best performing agent as the antagonist.
As long as any agent has a higher performance than the other agent, the objective will continue to improve the weakest agent.
During that time, the other agent in the policy continues learning, and therefore provide a stronger maximum performance against which we measure the regret. The Flexible PAIRED algorithm we propose is shown below. Using policy gradient updates, we train each agent in the population to optimize environmental reward, and the adversary to maximize the regret as computed in Eq. \ref{eq:flexible_regret}.

% \begin{algorithm}[H]
% % \SetAlgoLined
% \begin{algorithmic}[1]
%  \State \textbf{Input:}{$A,P$: Initialize two agents independently}
%  \State $W$ $\longleftarrow$ Run the adversary $\pi_E$ to generate a new website
%  \State $R_{A}$, $R_{P}$ $\longleftarrow$ Run agent $A$ and $\mathcal{P}$ in the environment $W$ for $M$ episodes and collect rewards
%  \State REGRET $\leftarrow \frac{1}{M} (\max_{\mathcal{A},\mathcal{P}} (\sum_{m=1}^M{R_{\mathcal{A}, m}}, \sum_{m=1}^M{R_{\mathcal{P}, m}}) - 0.5(\sum_{m=1}^M{R_{\mathcal{A}, m}} + \sum_{m=1}^M{R_{\mathcal{P}, m}}))$
%  \State Update adversary parameters using REGRET as the reward
%  \State Update parameters of $A$ and $\mathcal{P}$ using $R_{A,m}$ and $R_{\mathcal{P},m}$, respectively
% \end{algorithmic}
%  \caption{One step training of flexible PAIRED}
% \end{algorithm}

\begin{algorithm}[H]
% \SetAlgoLined
\begin{algorithmic}[1]
 \State \textbf{Input:}{$A,P$: Initialize two agents independently}
 \State $W$ $\longleftarrow$ Run the adversary $\pi_E$ to generate a new website
 \State $R^{A}$, $R^{P}$ $\longleftarrow$ Run agent $A$ and $P$ in the environment $W$ and collect rewards
 \State REGRET $\longleftarrow$ Compute regret as in Eq. \ref{eq:flexible_regret}
 \State Update adversary parameters using REGRET as the reward
 \State Update parameters of $A$ and $P$ using $R^{A}$ and $R^{P}$, respectively
\end{algorithmic}
 \caption{One step training of flexible PAIRED}
\end{algorithm}

\subsection{Budget Enforcing on Adversary}
Consider the following scenario where agents are placed on the home page of a shopping website where there are many possible elements, but only a single button that takes them to their account page.
During exploration, agents mostly collect negative rewards for taking incorrect actions, bounded to a very narrow interval (as there is only a single optimal action).
In this case, the regret is very small and non-informative, which hinders the adversary's ability to design environments at an appropriate difficulty for agents to learn.
This is true even with the proposed flexible regret objective.
% Intuitively, adversary should increase/decrease environment's difficulty only if antagonist agents 

To mitigate this problem, we use a budget enforcing objective in addition to the regret that binds the adversary's design budget to the performance of the best agent.
We approximate the effective budget of the adversary as the expected number of non-SKIP actions over $N$ time steps and update this budget according to whether the agents are learning.
More formally, we use the following minimization objective for budget enforcing that is added to the PAIRED objective:
\begin{equation}
    \mathcal{O}_{budget} = R^A * \sum_{i=1}^N{\log  \pi(a_i=\text{SKIP}|a_{0\cdots i-1}, b_{0,\cdots, i-1})}
\end{equation}
where $R^A$ is the reward of the antagonist (or the best-performing) agent.
This objective encourages the adversary to use less budget (more SKIP actions) when the agents are not yet learning (i.e.,  $R^A$ is negative or low); it encourages the adversary to use more budget (less SKIP actions) when the \webnav\ agents are collecting positive rewards in the environment.



==> src/realted_before_rebuttal.tex <==
\section{Related work}
Prior work on training agents to navigate the web introduced the Miniwob \citep{shi2017world} and Miniwob++ \citep{liu2018reinforcement} environments, but relied on obtaining expert demonstrations for each website, which cannot scale effectively to cover the large variety of real-world websites, and cannot adapt to changing websites. Further, these methods failed to solve complex web navigation tasks such as flight booking or social media interaction \citep{gur2018learning}. 
\citet{gur2018learning} take a step farther by training an RL agent to solve complex web navigation tasks using a scheduled curriculum. The curriculum linearly increases a parameter $p$, in which $1-p$ controls the number of web elements that are solved by querying an oracle policy, which is obtained via expert data. %In contrast, we do not rely on any expert demonstrations, and instead assume that we are given a set of (key, value) instructions, consisting of the values to enter for certain fields, such as \textit{username}.
%In contrast, we use AEG to automatically learn to generate a curriculum of web navigation tasks that are tailored to the current skill level of the agent. 
%Furthermore, we make no assumption on the availability of any website while they assume websites are given \textit{a priori}.
This work differs in several ways. First, we do not rely on any expert demonstrations to augment sparse rewards. We use AEG to automatically learn to generate a curriculum of web navigation tasks that are tailored to the current skill level of the agent. 
Next, we make no assumption on the availability of any website while they assume websites are given \textit{a priori}. Lastly, our web navigation agents generalize to unseen environments. 

Multi-agent training can be an effective method for automatically generating a curriculum of RL tasks (e.g. ~\citet{leibo2019autocurricula,matiisen2019teacher,graves2017automated,portelas2020teacher}). For example, Asymmetric Self Play (ASP) \citep{sukhbaatar2017intrinsic} trains two agents, in which the second agent must learn to repeat the actions taken by the first, demonstrator agent.
% Because the demonstrator cannot pose a task that it cannot complete itself, this technique ensures that each task proposed is feasible.
Both agents play in the same, fixed environment. In contrast, we use a third agent to learn to generate challenging new environments. 
POET \citep{wang2019paired,wang2020enhanced} %shows how a population of environment agents
is an AEG technique which uses a population of adversaries to generate the terrain a 2D walker agent must learn to navigate.
To create a curriculum, POET requires generating many new environments, testing all agents within each one, and discarding environments based on a manually chosen a reward threshold, which wastes a significant amount of computation. 
\citet{campero2020learning} use a teacher to propose navigation tasks; the teacher's reward is based on whether the agent takes more steps than a threshold, a hyperparmeter that is linearly increased over the course of training.
% In contrast with both of these works, we use a minimax regret training scheme which automatically learns to tailor the difficulty of proposed environments to the current skill level of the learner. 

Most closely related to our work is PAIRED \citep{dennis2020emergent}, which is an AEG method for training agents with minimal regret that works by constraining the environment-generating adversary using the performance of a second agent. However, PAIRED only demonstrated results on simple gridworld environments, and did not expand to the type of complex, high-dimensional state-action space required for web navigation. We improve on PAIRED using a more flexible estimate of the regret, as well as a budget mechanism, and show that this significantly improves performance.

%%%%%%%%%%%%%%%%%%%
%%Neural Programmer-Interpreters for learning hierarchical neural programs domain-specific encoders for different environments. \cite{reed2015neural, pierrot2019learning} 
%%%%%%%%%%%%%%%%%%%

==> src/related.tex <==
\vspace*{-0.1in}
\section{Related work}
\vspace*{-0.1in}
\textbf{Web navigation benchmarks and tasks:}
Prior work on training agents to navigate the web introduced the MiniWoB \citep{shi2017world} and MiniWoB++ \citep{liu2018reinforcement} environments, a fixed set of manually curated toy websites, but relied on obtaining expert demonstrations for each website, which cannot scale effectively to cover the large variety of real-world websites, and cannot adapt to changing websites. Further, these methods failed to solve complex web navigation tasks such as flight booking or social media interaction \citep{gur2018learning}. 
\citet{gur2018learning} take a step farther by training an RL agent to solve complex web navigation tasks using a scheduled curriculum. The curriculum linearly increases a parameter $p$, in which $1-p$ controls the number of web elements that are solved by querying an oracle policy, which is obtained via expert data. %In contrast, we do not rely on any expert demonstrations, and instead assume that we are given a set of (key, value) instructions, consisting of the values to enter for certain fields, such as \textit{username}.
%In contrast, we use AEG to automatically learn to generate a curriculum of web navigation tasks that are tailored to the current skill level of the agent. 
%Furthermore, we make no assumption on the availability of any website while they assume websites are given \textit{a priori}.
This work differs in several ways. First, we introduce a new framework, gMiniWoB, that allows generating complex websites on-the-fly with tunable difficulty levels. Additionally, we do not rely on any expert demonstrations to augment sparse rewards. We use AEG to automatically learn to generate a curriculum of web navigation tasks that are tailored to the current skill level of the agent. 
Next, we make no assumption on the availability of any website while they assume websites are given \textit{a priori}. Lastly, our web navigation agents generalize to unseen environments. 

\textbf{Goal Generation:} \citet{florensa18a} trains a Generative Adversarial Network (GAN) for generating a curriculum of goals with fixed environment dynamics.
A generator is trained to output new goals and the discriminator is trained to predict if the goal is achievable.
The generator is bootstrapped from sample goals that the initial agent is able to reach in the environment.
It is tested on simple navigation tasks with the same environments.
In contrast, we train an adversary that generates a curriculum of \textit{environments}, including goals, starting with an empty environment in which bootstrapping a generator network from sample episodes is not possible.
We test on unseen environments with more complicated and high dimensional state and action spaces.

\textbf{Adversarial Environment Generation:} Multi-agent training can be an effective method for automatically generating a curriculum of RL tasks (e.g. ~\citet{leibo2019autocurricula,matiisen2019teacher,graves2017automated,portelas2020teacher}). For example, Asymmetric Self Play (ASP) \citep{sukhbaatar2017intrinsic} trains two agents, in which the second agent must learn to repeat the actions taken by the first, demonstrator agent.
% Because the demonstrator cannot pose a task that it cannot complete itself, this technique ensures that each task proposed is feasible.
Both agents play in the same, fixed environment. In contrast, we use a third agent to learn to generate challenging new environments. 
POET \citep{wang2019paired,wang2020enhanced} %shows how a population of environment agents
is an AEG technique which uses a population of adversaries to generate the terrain a 2D walker agent must learn to navigate.
To create a curriculum, POET requires generating many new environments, testing all agents within each one, and discarding environments based on a manually chosen a reward threshold, which wastes a significant amount of computation. 
\citet{campero2020learning} use a teacher to propose navigation tasks; the teacher's reward is based on whether the agent takes more steps than a threshold, a hyperparameter that is linearly increased over the course of training.
% In contrast with both of these works, we use a minimax regret training scheme which automatically learns to tailor the difficulty of proposed environments to the current skill level of the learner. 

Most closely related to our work is PAIRED \citep{dennis2020emergent}, which is an AEG method for training agents with minimal regret that works by constraining the environment-generating adversary using the performance of a second agent. However, PAIRED only demonstrated results on simple gridworld environments, and did not expand to the type of complex, high-dimensional state-action space required for web navigation. We improve on PAIRED using a more flexible estimate of the regret, as well as a budget mechanism, and show that this significantly improves performance.

\textbf{RL with Autoregressive Models:} \citet{seq2seqrl} outlines training sequence-to-sequence (seq2seq) models with RL algorithms.
Previous models first pretrained a seq2seq model with ground-truth inputs and outputs and then finetuned with RL using different reward functions such as BLEU score.
In this work, we propose a decoder-like autoregressive adversary model that is trained without any ground-truth data.
The model is fed its own predictions from previous time steps and updated using a novel adversarial objective.
%%%%%%%%%%%%%%%%%%%
%%Neural Programmer-Interpreters for learning hierarchical neural programs domain-specific encoders for different environments. \cite{reed2015neural, pierrot2019learning} 
%%%%%%%%%%%%%%%%%%%
